Which Identities Are Mobilized: Towards an automated detection of social group appeals in political texts

This paper proposes a computational text classification strategy to identify references to social groups in European party manifestos and beyond. Our methodology uses machine learning techniques, including BERT and large language models, to capture group-based appeals in texts. We propose to combine automated identification of social groups using the Mistral-7B-v0.1 Large Language Model with Embedding Space-based filtering to extend a sample of core social groups to all social groups mentioned in party manifestos. By applying this approach to RRP's and mainstream parties' group images in manifestos, we explore whether electoral dynamics explain similarities in group appeals and potential convergence or divergence in party strategies. Contrary to expectations, increasing RRP support or mainstream parties' vote loss does not necessarily lead to convergence in group appeals. Nonetheless, our methodology enables mapping similarities in group appeals across time and space in 15 European countries from 1980 to 2021 and can be transferred to other use cases as well.

==> content/0A1_Tables_Figures/plausitab.tex <==
% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sat, May 06, 2023 - 14:07:05
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{plausi} 
\footnotesize 
\begin{tabular}{@{\extracolsep{5pt}} llll} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Category & Plausible & Recoded to zero & Number of Tweets after coding \\ 
\hline \\[-1.8ex] 
External Relations & 349 (69.8\%) & 115 (76.16\%) & $396$ \\ 
Freedom and Democracy & 340 (68\%) & 101 (63.12\%) & $377$ \\ 
Political System & 239 (47.8\%) & 193 (73.95\%) & $262$ \\ 
Economy & 385 (77\%) & 57 (49.57\%) & $442$ \\ 
Fabric of Society & 335 (67\%) & 131 (79.39\%) & $383$ \\ 
Social Groups & 375 (75\%) & 98 (78.4\%) & $399$ \\ 
EU & 309 (61.8\%) & 144 (75.39\%) & $343$ \\ 
Technology and Infrastructure & 352 (70.4\%) & 116 (78.38\%) & $394$ \\ 
Environmental Protection & 412 (82.4\%) & 66 (75\%) & $458$ \\ 
Education and Culture & 330 (66\%) & 142 (83.53\%) & $351$ \\ 
Social welfare and Equality & 403 (80.6\%) & 52 (53.61\%) & $468$ \\ 
Migration & 335 (67\%) & 118 (71.52\%) & $395$ \\ 
Zero category & NA (NA\%) & NA (NA\%) & $1,331$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 

==> content/0A1_Tables_Figures/regression.tex <==
% Date and time: Sat, May 06, 2023 - 14:22:31
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
\\[-1.8ex] &  \\ 
 & Vote Thief \\ 
\hline \\[-1.8ex] 
 vote\_thief\_dummy1 & 0.121 \\ 
  & (1.537) \\ 
  & \\ 
 lost\_votes\_total & $-$0.003 \\ 
  & (0.758) \\ 
  & \\ 
 Constant & $-$0.006 \\ 
  & (0.511) \\ 
  & \\ 
\hline \\[-1.8ex] 
Observations & 234 \\ 
R$^{2}$ & 0.00003 \\ 
Adjusted R$^{2}$ & $-$0.009 \\ 
Residual Std. Error & 5.753 (df = 231) \\ 
F Statistic & 0.003 (df = 2; 231) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> content/0B-disclaimer.tex <==
\begin{center} % Center text
    Word count: XXXX
% How to check words in a LaTeX document: https://www.overleaf.com/help/85-is-there-a-way-to-run-a-word-count-that-doesnt-include-latex-commands
\end{center}

==> content/0C-toc.tex <==
%---------------------------------------------------------------------------------
% Table of content
%---------------------------------------------------------------------------------

%\newpage % Generates page break

% Table of content
\thispagestyle{empty} % Suppresses page numbers
\tableofcontents % Adds table of content
\newpage % Generates page break

% List of figures
\thispagestyle{empty} % Suppresses page numbers
\listoffigures % Adds list of figures; uncomment if required
\newpage % Generates page break; uncomment if required

% List of tables
\thispagestyle{empty} % Suppresses page numbers
\listoftables % Adds list of tables; uncomment if required
\newpage % Generates page break; uncomment if required


==> content/9B-declaration.tex <==
%----------------------------------------------------------------------------------------
% Declaration
%----------------------------------------------------------------------------------------
\newpage % Includes a page break
\thispagestyle{empty} % Leaves the page style empty (no page number, no header, no footer)
\section*{Statutory Declaration} % Stars disable section numbers

\begin{otherlanguage}{german}
Hiermit versichere ich, dass diese Arbeit von mir pers\"{o}nlich verfasst ist und dass ich keinerlei fremde Hilfe in Anspruch genommen habe. Ebenso versichere ich, dass diese Arbeit oder Teile daraus weder von mir selbst noch von anderen als Leistungsnachweise andernorts eingereicht wurden. W\"{o}rtliche oder sinngem\"{a}{\ss}e \"{U}bernahmen aus anderen Schriften und Ver\"{o}ffentlichungen in gedruckter oder elektronischer Form sind gekennzeichnet. S\"{a}mtliche Sekund\"{a}rliteratur und sonstige Quellen sind nachgewiesen und in der Bibliographie aufgef\"{u}hrt. Das Gleiche gilt f\"{u}r graphische Darstellungen und Bilder sowie f\"{u}r alle Internet-Quellen. Ich bin ferner damit einverstanden, dass meine Arbeit zum Zwecke eines Plagiatsabgleichs in elektronischer Form anonymisiert versendet und gespeichert werden kann. Mir ist bekannt, dass von der Korrektur der Arbeit abgesehen und die Pr\"{u}fungsleistung mit nicht ausreichend bewertet werden kann, wenn die Erkl\"{a}rung nicht erteilt wird.
\end{otherlanguage}

\vspace*{1in} % Adds extra space between two paragraphs

\noindent I hereby declare that the paper presented is my own work and that I have not called upon the help of a third party. In addition, I affirm that neither I nor anybody else has submitted this paper or parts of it to obtain credits elsewhere before. I have clearly marked and acknowledged all quotations or references that have been taken from the works of others. All secondary literature and other sources are marked and listed in the bibliography. The same applies to all charts, diagrams and illustrations as well as to all Internet resources. Moreover, I consent to my paper being electronically stored and sent anonymously in order to be checked for plagiarism. I am aware that the paper cannot be evaluated and may be graded ``failed'' (``nicht ausreichend'') if the declaration is not made.\\

%\vspace*{1in} % Adds extra space

% Add field for signature, date, and place
\hfill \signature{} 

